Contact angles on a soft solid: from Young's law to Neumann's law

The contact angle that a liquid drop makes on a soft substrate does not obey the classical Young's relation, since the solid is deformed elastically by the action of the capillary forces. The finite elasticity of the solid also renders the contact angles different from that predicted by Neumann's law, which applies when the drop is floating on another liquid. Here we derive an elasto-capillary model for contact angles on a soft solid, by coupling a mean-field model for the molecular interactions to elasticity. We demonstrate that the limit of vanishing elastic modulus yields Neumann's law or a slight variation thereof, depending on the force transmission in the solid surface layer. The change in contact angle from the rigid limit (Young) to the soft limit (Neumann) appears when the length scale defined by the ratio of surface tension to elastic modulus $\gamma/E$ reaches a few molecular sizes.

==> LetterEditor.tex <==
Dear Editor,
In this submitted manuscript we answer a fundamental question of wetting: what is the contact angle that a liquid makes on a soft, deformable substrate.

The contact angle is usually determined from two classical wetting laws: valid either for stiff solid substrates (perfectly rigid) or for liquid substrates (perfectly soft). However, many recent studies in physics and materials science deal with intermediate cases, where the capillary interactions of the liquid are comparable to the elasticity of the substrate. Our work for the first time reveals the boundary condition at the three-phase contact line for substrates of arbitrary softness, which results from an intricate coupling of molecular interactions and elasticity.


As possible referees we would like to suggest:

Pedro Reis (MIT), Bob Evans (Bristol), Lyderic Bocquet (Lyon), Martin Brinkmann (Goettingen), Christophe Clanet (Ecole Polytechnique, ParisTech), Michael Brenner (Harvard), Arezki Boudaoud (Lyon) Stephen Wilson (Strathclyde, Glasgow).

Due to conflicting interests, we would prefer if Eric Dufresne (Yale) is not consulted for review.

